Formal Verification of Probabilistic SystemC Models with Statistical Model Checking

Transaction-level modeling with SystemC has been very successful in describing the behavior of embedded systems by providing high-level executable models, in which many of them have inherent probabilistic behaviors, e.g., random data and unreliable components. It thus is crucial to have both quantitative and qualitative analysis of the probabilities of system properties. Such analysis can be conducted by constructing a formal model of the system under verification and using Probabilistic Model Checking (PMC). However, this method is infeasible for large systems, due to the state space explosion. In this article, we demonstrate the successful use of Statistical Model Checking (SMC) to carry out such analysis directly from large SystemC models and allow designers to express a wide range of useful properties. The first contribution of this work is a framework to verify properties expressed in Bounded Linear Temporal Logic (BLTL) for SystemC models with both timed and probabilistic characteristics. Second, the framework allows users to expose a rich set of user-code primitives as atomic propositions in BLTL. Moreover, users can define their own fine-grained time resolution rather than the boundary of clock cycles in the SystemC simulation. The third contribution is an implementation of a statistical model checker. It contains an automatic monitor generation for producing execution traces of the model-under-verification (MUV), the mechanism for automatically instrumenting the MUV, and the interaction with statistical model checking algorithms.

==> appA.tex <==
\section*{Appendix: The Running Example Implementation}
\label{sec:appA}
\subsection*{The SystemC Source Code}
\begin{lstlisting}[caption=The fifo\_if.h,label=lst:fifointerfaces,mathescape]
#ifndef FIFO_IF
#define FIFO_IF
#include <systemc.h>

class fifo_write_if : virtual public sc_interface {
public:
   virtual void fifo_write(char) = 0;
   virtual void fifo_reset() = 0;	
};

class fifo_read_if : virtual public sc_interface {
public:
   virtual void fifo_read(char&) = 0;
   virtual int fifo_num_available() = 0;
};

#endif
\end{lstlisting}
\begin{lstlisting}[caption=The fifo.cpp,label=lst:fifo,mathescape]
#ifndef BASE_CHANNEL_H
#define BASE_CHANNEL_H
#include <systemc.h>
#include "fifo_if.h"

class Fifo : public sc_channel, public fifo_write_if, public fifo_read_if {
private:
   enum e {max = 10}; // capacity of the fifo
   char data[max];
   int num_elements, first;
   sc_event write_event, read_event;

public:
   Fifo(sc_module_name name) : sc_channel(name), num_elements(0), first(0) {}
   
   void fifo_write(char c) {
      if (num_elements == max) {
         wait(read_event);
      }

      data[(first + num_elements) % max] = c;
      ++num_elements;
      write_event.notify();
   }

   void fifo_read(char &c) {
      if (num_elements ==  0) {
         wait(write_event);
      }
		
      c = data[first];
      --num_elements;
      first = (first + 1) % max;
      read_event.notify();
   }

   void fifo_reset() {
      num_elements = 0;
      first = 0;
   }

   int fifo_num_available() {
      return num_elements;
   }
};

#endif
\end{lstlisting}
\begin{lstlisting}[caption=The consumer.h,label=lst:consumerh,mathescape]
#ifndef CONSUMER_H
#define CONSUMER_H

#include <systemc.h>
#include <tlm.h>
#include "fifo.cpp"
#include "utils.h"
#include <gsl/gsl_rng.h>
#include <gsl/gsl_randist.h>
#include <gsl/gsl_cdf.h>

SC_MODULE(Consumer) {
   SC_HAS_PROCESS(Consumer);
public:
   // Definitions of ports
   sc_port<fifo_read_if> in; // input port
   // Constructor
   Consumer(sc_module_name name, int c_init, gsl_rng *rnd);
   // Destructor
   ~Consumer() {};
   // Definition of processes
   void main();
   // Reading function
   void receive(char &c);

private:
   // Reading character in ASCII
   int c_int;
   gsl_rng *r;
};

#endif
\end{lstlisting}
\begin{lstlisting}[caption=The consumer.cpp,label=lst:consumercpp,mathescape]
#include "consumer.h"

Consumer::Consumer(sc_module_name name, int c_init, gsl_rng *rnd) {
   c_int = c_init;
   r = rnd; // random generator
 
   SC_THREAD(main);
}

void Consumer::receive(char &c) {
   in->fifo_read(c);
   c_int = c;
}

void Consumer::main() {
   char c;
   while (true) {
      // use the Bernoulli distribution in GSL
      int b = get_bernoulli(r,0.90);
      if (b) {
         receive(c);
      }
	
      wait(1,SC_NS); // waits for 1 nanosecond
   }	
}
\end{lstlisting}
\begin{lstlisting}[caption=The producer.h,label=lst:producerh,mathescape]
#ifndef PRODUCER_H
#define PRODUCER_H

#include <systemc.h>
#include <tlm.h>
#include "fifo.cpp"
#include "utils.h"
#include <gsl/gsl_rng.h>
#include <gsl/gsl_randist.h>
#include <gsl/gsl_cdf.h>

SC_MODULE(Producer) {
   SC_HAS_PROCESS(Producer);
public:
   // Definitions of ports
   sc_port<fifo_write_if> out; // output port
   // Constructor
   Producer(sc_module_name name, int c_init, gsl_rng *rnd);
   // Destructor
   ~Producer() {};
   // Definition of processes
   void main();
   // Writing function
   void send(char c);

private:
   int c_int;
   gsl_rng *r;
};

#endif
\end{lstlisting}
\begin{lstlisting}[caption=The producer.cpp,label=lst:producercpp,mathescape]
#include "producer.h"

Producer::Producer(sc_module_name name, int c_init, gsl_rng *rnd) {
   c_int = c_init;
   r = rnd; // random generator

   SC_THREAD(main);
}

void Producer::send(char c) {
	out->fifo_write(c);
	c_int = c;
}

void Producer::main() {
   const char* str = "&abcdefgh@";
   const char* p = str;
   while (true) {
      int b = get_bernoulli(r,0.90);
      if (b) {
         send(*p);
         p++;
         if (!*p) {
            p = str;
         }
      }
      wait(1,SC_NS); // waits for 1 nanosecond
   }	
}
\end{lstlisting}
\begin{lstlisting}[caption=The main.cpp,label=lst:main,mathescape]
#include <time.h>
#include "fifo.cpp"
#include "consumer.h"
#include "producer.h"

#include <gsl/gsl_rng.h>
#include <gsl/gsl_randist.h>
#include <gsl/gsl_cdf.h>
// The monitor generated by MAG
#include "monitor.h"

int sc_main(int argc, char *argv[]) {
   // random generator in GSL
   const gsl_rng_type *T;
   gsl_rng *r;
   gsl_rng_env_setup();
   T = gsl_rng_default;
   r = gsl_rng_alloc(T);
   // seed the generator
   srand(time(NULL));
   gsl_rng_set(r,random());
 
   sc_set_time_resolution(1,SC_NS); // time unit
   Fifo afifo("fifo"); // create a channel fifo
   Producer prod("producer",-1,r);
   Consumer cons("consumer",-1,r);
   prod.out(afifo); // the producer binding
   cons.in(afifo);  // the consumer binding
   // the observer for Instrumented model
   mon_observer* obs = local_observer::createInstance(1, 
                       &cons, 
                       &prod);
   sc_start();
   gsl_rng_free (r); // release the generator
   return 0;
}
\end{lstlisting}
\subsection*{Observed Variables, Temporal Resolution, and Properties}
\begin{lstlisting}[caption=The configuration file for MAG,label=lst:configurationfile,mathescape]
# Where to output the monitor
output_file   ./monitor.cpp

# The (class) name of the generated monitors
mon_name   monitor

# Plasma project file
plasma_file   /PLASMA_Lab-1.3.0/fifo/fifo.plasma

# Plasma project name
plasma_project_name   fifo

# Plasma model name
plasma_model_name   fifo_model

# Instrumented executable SystemC model
plasma_model_content   /PLASMA_Lab-1.3.0/fifo/fifo

# Set to write traces to a file
write_to_file   false

# Declare monitors as friend to adder class
usertype   Consumer
usertype   Producer

# Example of how to declare type of non-native variables
type Consumer   *pnt_con
type Producer   *pnt_pro

# Module attributes
attribute pnt_con->c_int   c_read
attribute pnt_pro->c_int   c_write

# Attribute type
att_type int   c_read
att_type int   c_write
att_type int   n_elements

# Time resolution
time_resolution   MON_TIMED_NOTIFY_PHASE_END

# Properties
formula G<=#10000((c_read = 38) => (F<=#15(c_read = 64)))

# Includes the files
include consumer.h
include producer.h
\end{lstlisting}


==> appB.tex <==
\section*{Appendix B: Additional Experimental Results}
\label{sec:appB}
In addition to the analysis in \secref{subsec:ecs}, we study the probability that each of the four types of failure eventually occurs in the first $T$ time of operation. This is done using the BLTL formula $F_{\leq T} \; (failure_i)$.
%------------------------------%
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.90\textwidth]{figs/eachfailure.png}
\caption{The probability that each of the 4 failure types in the first $T$ time of operation}
\label{fig:failure}
\end{center}
\end{figure}
%------------------------------%
%------------------------------%
\begin{figure}[ht]
\centering
\includegraphics[width=0.90\textwidth]{figs/numberreboot.png}
\caption{Expected number of reboots that occur in the first $T$ time of operation}
\label{fig:numberofreboots}
\end{figure}
%------------------------------%
%------------------------------%
\begin{figure}[ht]
\centering
\includegraphics[width=0.90\textwidth]{figs/numberworking.png}
\caption{Expected number of functional sensor and actuator groups in the first $T$ time of operation}
\label{fig:numberofworkinggroups}
\end{figure}
%------------------------------%
\figref{fig:failure} plots these probabilities over the first $30$ days of operation. We observe that the probabilities that the sensors and I/O processors eventually fail are more than the others do. In the long run, they are almost the same and approximate to $1$, meaning that the sensors and I/O processors will eventually fail with probability $1$. The main processor has the smallest probability to eventually fail.

Finally, we approximate the number of reboots of the I/O processors, and the number sensor groups, actuator groups that are functional over time by computing the expected values of random variables that count the number of reboots, functional sensor and actuator groups. The results are plotted in Fig. \ref{fig:numberofreboots} and Fig. \ref{fig:numberofworkinggroups}. It is obvious that the number of reboots of both processors doubles the number of reboots of each processor since they have the same behavior.

